Small But Funny: A Feedback-Driven Approach to Humor Distillation

The emergence of Large Language Models (LLMs) has brought to light promising language generation capabilities, particularly in performing tasks like complex reasoning and creative writing. Consequently, distillation through imitation of teacher responses has emerged as a popular technique to transfer knowledge from LLMs to more accessible, Small Language Models (SLMs). While this works well for simpler tasks, there is a substantial performance gap on tasks requiring intricate language comprehension and creativity, such as humor generation. We hypothesize that this gap may stem from the fact that creative tasks might be hard to learn by imitation alone and explore whether an approach, involving supplementary guidance from the teacher, could yield higher performance. To address this, we study the effect of assigning a dual role to the LLM - as a "teacher" generating data, as well as a "critic" evaluating the student's performance. Our experiments on humor generation reveal that the incorporation of feedback significantly narrows the performance gap between SLMs and their larger counterparts compared to merely relying on imitation. As a result, our research highlights the potential of using feedback as an additional dimension to data when transferring complex language abilities via distillation.

==> figures/datasize.tex <==
    \begin{tikzpicture}[scale = 0.9]
\begin{axis}[
    xlabel=$N_{samples}$,
    ylabel=$BWR$,
    xmin=0, xmax=20,
    ymin=0, ymax=100,
    xtick={0,10,20},
    xticklabels={12K,24K,36K},   % <---
    ytick={0,10,...,100}
            ]
\addplot[smooth,mark=*,blue] plot coordinates {
    (0,26)
    (10,28)
    (20,37)
};
\addlegendentry{Without Feedback}

\addplot[smooth,color=red,mark=x]
    plot coordinates {
    (0,53)
    (10,59)
    (20,65)
    };
\addlegendentry{With Feedback}
\end{axis}
\label{fig:datasize}

    \end{tikzpicture}

==> figures/supervision.tex <==
    \begin{tikzpicture}[scale = 0.9]
\begin{axis}[
    xlabel=$N_{samples}$,
    ylabel=$BWR$,
    xmin=0, xmax=20,
    ymin=0, ymax=100,
    xtick={0,10,20},
    xticklabels={100, 50, 10},   % <---
    ytick={0,10,...,100}
            ]

\addplot[smooth,color=red,mark=x]
    plot coordinates {
    (0,46)
    (10,48)
    (20,60)
    };
\addlegendentry{With Feedback}
\end{axis}
    \end{tikzpicture}

==> sections/0-abstract-old.tex <==
Humor generation and understanding is a crucial step towards making AI agents more relatable and engaging in human interactions. Generating humor is a complex endeavor, demanding a profound understanding of language and commonsense knowledge. While Large Language Models (LLMs) have shown promise in generating funny text and jokes, there is a substantial performance gap when transferring such creative abilities to smaller models. Previous work has indicated that imitation may be insufficient, as it does not address disparities in task comprehension and reasoning abilities. We hypothesize that this gap may stem from the static nature of imitation, particularly the absence of feedback between the teacher (LLM) and the student (smaller model). To address this, we study the effect of assigning a dual role to the LLM - as a \emph{teacher} generating data, as well as a \emph{critic} that evaluates performance on the humor generation task. Our experiments reveal that the preference data from the teacher helps in aligning the student to the desired level of humor, leading to a significant improvement in performance compared to simple imitation. Our research highlights the potential of using feedback as an additional dimension to data when transferring creative language abilities via distillation.



% We hypothesize that this gap may stem from the static nature of imitation, particularly the absence of feedback between the teacher (LLM) and the student (smaller model).

==> sections/1-intro-old.tex <==
Integrating humor into language agents fosters more natural and engaging conversations, making them more appealing to users \cite{Ritchie2007APA}.  With the advent of Large Language Models \cite{Touvron2023Llama2O, openai2023gpt4}, trained on diverse dialogue-style data and aligned with human preferences,  researchers have explored the generation of humor and creative assistance using language models \cite{Chakrabarty2023CreativitySI, Chen2023ProbingTC}. Large Language Models (LLMs) exhibit varying degrees of success in generating humorous content. While LLMs do not match the subtleties of humor in human-written text \cite{hessel-etal-2023-androids, Chakrabarty2023ArtOA}, larger models demonstrate better creative generation and understanding abilities compared to their smaller counterparts \cite{Radford2019LanguageMA, chen2023minigptv2, hessel-etal-2023-androids}. Larger models achieve this by learning humor patterns from vast amounts of diverse textual data, enabling them to recognize and replicate certain comedic structures. 

% How do smaller LMs like BART do and why do they not reach similar levels of creativity as LLMs?
Smaller language models \cite{lewis-etal-2020-bart,zhang2022opt, Radford2019LanguageMA} may not exhibit similar levels of creativity as their larger counterparts due to differences in model size and amount of training data. While these models may excel in tasks such as abstractive summarization and paraphrasing \cite{lewis-etal-2020-bart}, they tend to prioritize fidelity to input content over creative generation. The depth of understanding and the ability to relate concepts playfully or unexpectedly is correlated with the amount of information and examples the model has been exposed to, which is typically lower in smaller LMs.

% Can we distill this ability by training on LLM's humorous outputs?
In this work, we investigate whether the ability to generate humor can be distilled from LLMs into smaller models by performing task-specific knowledge-distillation \cite{west-etal-2022-symbolic} - i.e. training smaller student models on data curated from the responses of larger teacher models. This transfer learning could allow smaller models to adopt patterns of humor by imitating patterns from the teacher. However, the distillation of data through Large Language Models (LLMs) raises issues related to the transferability of knowledge, particularly when attempting to teach smaller models about the task of generating humor — a complex and nuanced aspect of language \cite{mukherjee2023orca, gudibande2023false}. 




Recent work has demonstrated the success of LLMs in providing evaluation scores or natural language feedback on generative tasks \cite{Shinn2023ReflexionLA, akyurek-etal-2023-rl4f, Madaan2023SelfRefineIR}. Building upon the capabilities of Large Language Models (LLMs) as evaluators, we investigate whether preference data from the teacher could be harnessed to guide the distillation of complex language abilities such as humor generation. We adopt a straightforward yet robust approach to feedback, utilizing pairwise scoring to provide nuanced guidance to the smaller student model.  Through human evaluation, we critically assess the strengths and limitations of the teacher in evaluating the student. Our experiments reveal that, the student trained on preference data with positive and negative demonstrations performs significantly better than the student trained on positive demonstrations alone. We further investigate the following research questions on the nature and frequency of teacher intervention:
\begin{enumerate}[label=\large\protect\textcircled{\small\arabic*}]
\item  What is the effect of data size on student performance? \sahi{Answer (Section 6): Improves performance with and without feedback}
\item How often is the intervention from the teacher required to cause significant improvements in student performance?
\sahi{Answer (Section 6): More frequent intervention improves win rates, but at the cost of communication}
\item How do biases in model-based evaluation affect student behavior while incorporating feedback? 
\sahi{Answer  (Section 6): Biases in length reflect in student response length increasing as we train for more time over preferences: We filtered equal length training and use length penalties during generation to mitigate this. However, this motivates future work on reducing length bias in preference learning.}
% \item Is the source of preference candidate (e.g. teacher vs. student) shown during training important in influencing performance?
\end{enumerate}


% We highlight the need for more dynamic teacher-student communication when distilling complex language abilities and approaches to mitigate biases in evaluation.





% Additionally, we explore whether the feedback from the critic could be leveraged to effectively guide the student model toward producing more humorous outputs. 
%  % We leverage contrastive training for students from the sequence-sequence student family and the DPO method for the decoder-only model family.
% We found that irrespective of the student architecture as well as the incorporation method used for feedback, the student trained on positive and negative demonstrations can go on to match the teacher performance under LLM-based (critic) evaluation. Furthermore, we show that the student models that leverage feedback guidance perform significantly better in human evaluation than the students trained on data distillation. However, our human evaluation highlights that humans still prefer the response of the LLM higher than the output of both data/feedback driven student models, indicating the 
% potential for improvements in LLM-based evaluation. 

% We observed that regardless of the student architecture and the feedback incorporation method employed, training the student using both positive and negative demonstrations consistently enables it to achieve performance levels comparable to the teacher under LLM-based (critic) evaluation. Additionally, our findings reveal a notable performance advantage for student models guided by feedback compared to those trained through data distillation when evaluated by human assessors. Despite this, our human evaluation indicates a preference for responses generated by the LLM over outputs from both data-driven and feedback-driven student models, signaling room for further enhancements in LLM-based evaluation





% Our analysis
% reveals both the benefits and risks of the LLMas-reference setting. On the one hand, smaller
% models can indeed benefit from LLM’s guidance
% and the contrastive learning method. On the other
% hand, LLM-based evaluation fails to align with human evaluation since human evaluation still prefers
% LLMs over smaller models, while they achieve similar performance under LLM-based evaluation.

% \begin{enumerate}[label=\large\protect\textcircled{\small\arabic*}]
% \item  What is the effect of data size on student performance? \sahi{Answer (Section 6): Improves performance with and without feedback}
% \item How often is the intervention from the teacher required to cause significant improvements in student performance?
% \sahi{Answer (Section 6): More frequent intervention improves win rates, but at the cost of communication}
% \item How do biases in model-based evaluation affect student behavior while incorporating feedback? 
% \sahi{Answer  (Section 6): Biases in length reflect in student response length increasing as we train for more time over preferences: We filtered equal length training and use length penalties during generation to mitigate this. However, this motivates future work on reducing length bias in preference learning.}
% % \item Is the source of preference candidate (e.g. teacher vs. student) shown during training important in influencing performance?
% \end{enumerate}


